LibriBrain: Over 50 Hours of Within-Subject MEG to Improve Speech Decoding Methods at Scale

LibriBrain represents the largest single-subject MEG dataset to date for speech decoding, with over 50 hours of recordings -- 5$\times$ larger than the next comparable dataset and 50$\times$ larger than most. This unprecedented `depth' of within-subject data enables exploration of neural representations at a scale previously unavailable with non-invasive methods. LibriBrain comprises high-quality MEG recordings together with detailed annotations from a single participant listening to naturalistic spoken English, covering nearly the full Sherlock Holmes canon. Designed to support advances in neural decoding, LibriBrain comes with a Python library for streamlined integration with deep learning frameworks, standard data splits for reproducibility, and baseline results for three foundational decoding tasks: speech detection, phoneme classification, and word classification. Baseline experiments demonstrate that increasing training data yields substantial improvements in decoding performance, highlighting the value of scaling up deep, within-subject datasets. By releasing this dataset, we aim to empower the research community to advance speech decoding methodologies and accelerate the development of safe, effective clinical brain-computer interfaces.

==> 3.0_notes.tex <==
{\color{red}

NOTES
\begin{itemize}
    \item Big data is defined as ... (relative term, but bigger than usual? -- what's usual here?)
    \item In neuroimaging, deep data is big data acquired within an individual
    \item Previously, the biggest similar data was Armeni: 10 hours for one Sherlock book
    \item We recorded $\sim$50 hours of SQUID-MEG from one subject, listening to the first 5--6 Sherlock books (chronologically in the canon) and 5\% of the clean LibriSpecech train, dev, and test sets
    \item All audio ultimately come from LibriVox...
    \item LibriSpeech data are excerpts from XXX stories, with XXX speakers
    \item To balance this, we included 5--6 Sherlock books all read by the same speaker (David Clarke)
    \item We provide a standard data split, which takes into account leakage (e.g.~holdout data, including val, test, and competition splits, all acquired on seperate days than any training data) -- more like use case than using some data from same day, and definitely not from slices between train data (see paper on correlations from Zeb)
    \item Holdout data are LibriSpeech test-clean data, Sherlock1 chapters 12 (test); 13 and 14 heldout for competition
    \item Validation data are Sherlock1 chapter 11 and LibriSpeech test-dev
    \item To simplify task for ML community in the first instance, we release serialised data, so that they can be thought of as tensors
    \item We plan to release BIDS format data at a later date / concurrently?
    \item Data are provided in sensor space
    \item We used a XXX scanner with 306 sensors (102 magnetometers, 204 gradiometers)
    \item These are arranged as in TODO: add schematic of sensor layout in Dewar
    \item TODO: add schematic of scanner
    \item We provide a data loader with an events file with time stamps for different events in the dataset
    \item For example (for the competition), we can load speech and non-speech for speech detection and 39 English phonemes for phoneme classification
    \item We manually corrected the text for text normalisation
    \item We used forced-alignment to find events in audio files and manually checked them
    \item We provide baseline models for speech detection and phoneme classification, showing that there is signal in the data and comparing it to prior datasets (Armeni, Gwilliams)
    \item We also include data loaders for these other datasets (as well as others); we show best results for training and evaluating only on LibriBrain data, and for training on Libribray plus more datasets and then evaluating on Libribrain test splits
    \item We hope taht by standardising evaluation we can better measure progress in the field, rather than just random splits datasets as in current practice with few exceptions (cf.~MegNIST?)
\end{itemize}
}


==> 4.1_subject.tex <==
\subsection{Participants}\label{sec:participants}


{\color{red}
\begin{itemize}
    \item In v1, 1 subj
    \item Say why: decoding better within subject (cite Richard paper, etc)
    \item We aim to include additional subjects in future releases
\end{itemize}
}


==> 5.4_metrics.tex <==
\subsection{Metrics}

\begin{itemize}
    \item There are many metrics that could be used
    \item For speech detection, we opt for IoU (see Slack for reasons)
    \item ...
    \item For phoneme classification, we report the following:
    \begin{itemize}
        \item Macro F1-Score (F1)
        \item Macro Precision
        \item Macro Recall
        \item Per-Class Precision (sensitive to false positives, so low precision indicates the model is frequently misclassifying other classes as this class)
        \item Per-Class Recall (more sensitive to false negatives, so low recall indicates the model is missing instances of a class)
        \item Confusion Matrix
    \end{itemize}
    \item The main metric we track is F1
    \item We use the Macro F1-Score variant, as it encourages improvements in the worst performing classes (rather than prioritising continued improvements in the most frequent classes)
    \item We might have preferred Weighted F1-Score for production purposes, as this first advances performance on the highest frequency phonemes (What does this mean? -M) 
    \item In the limit, either variety will converge on 100\% for each phoneme
    \item But we argue that we should reward advances on the harder classes first, to drive progress %
    \item Highlights performance on under-represented or difficult classes
    \item We will also track Weighted F1-Scores, to compare if different teams would have won...
    \item Macro F1 is calculated by computing F1 scores for each class independently, then taking the unweighted average of these scores across all classes
    \item Suppose we have two classes with F1 scores of 0.8 and 0.7, the macro F1 would be 7.5 = (0.8 + 0.7)/2
    \item Macro precision and recall help to explain what is happening in general...
    \item Per-Class recall is useful for seeing how many true cases are predicted
\end{itemize}



==> XXX_TODO <==

\subsection*{TODO: stimuli to collect}
\begin{enumerate}
    {\color{green}
    \item Sherlock 3 - done
    \item Sherlock 1 - done
    \item Sherlock 2 - done
    }
    {\color{blue}
    \item Sherlock 4 - in progress
    \item TODO: Sherlock 5
    \item TODO: Sherlock 6 (about 12 hrs, total about 46 hrs without LibriSpeech data, so add another 4 hours of that?)
    \item TODO: LibriSpeech test-clean (5\% is 15 minutes) %10\% is 0.5 hrs
    \item TODO: LibriSpeech dev-clean (5\% is 15 minutes) %10\% is 0.5 hrs
    \item TODO: LibriSpeech train-clean (5\% is 5 hrs)
    }
    {\color{orange} 
    \item NB: 100\% LibriSpeech test-clean (5 hrs)
    \item NB: 10\% to 100\% dev-clean (0.5 to 5 hrs)
    \item NB: 10\% train-clean-100 (10 hrs)
    }
    {\color{red} 
    \item NB: 2x time to collect repeat tasks (LibriSpeech), so 20 hrs listen should take 40 hours listen/think
    \item NB: if approx 1 hr LibriSpeech per scan, then plan for 40 LibriSpeech scans for 20 listen hrs
    }
    {\color{gray}
    \item Optional: Sherlock 4
    \item Optional: Sherlock 5
    }
\end{enumerate}


%
\begin{itemize}
    \item Audio from LibriSpeech dataset
    \item In v1:
    \begin{itemize}
        \item test-clean (5.4 hours total?) 100\% = 5.4 hrs (\textbf{half from sessions without dev or train trials; half for sessions/runs with dev and train trials mixed in}) %to control for question of whether any leakage? or if scan on different day matters?
        \item dev-clean (5.4 hours total?) 10\% = 0.54 hrs for validation
        \item train-clean-100 (100 hours total?) 10\% = 10 hrs (\textbf{TOTAL = approx 16 hours -> x2 for listen/repeat = 32 hrs})
        \item {\color{gray} OR: train-clean-100 20\% = 20 hrs?? (TOTAL = approx 26 hours - x2 for listen/repeat = 52 hrs!)}
    \end{itemize}
    \item Since LibriSpeech sentences are mostly out of context, we also wanted to collect some extended narratives
    \item We note Armeni as best prior dataset, which has recordingsn for 3 subjects doing 10 hours of Sherlock3
    \item We also include approx 20--34 hours of Sherlock books from LibriVox ({\color{red} TODO(check): any overlap with LibriSpeech test?})
    \begin{enumerate}
        \item A Study in Scarlet (1887), {\color{red} 04:37:34?}
        \item The Sign of the Four (1890), {\color{red} 4:27:31?}
        \item The Adventures of Sherlock Holmes (1892), {\color{blue} 12 stories}, {\color{red} 10:56:13?}
        {\color{gray}
        \item The Memoirs of Sherlock Holmes (1893--1894), {\color{blue} 12 stories}, {\color{red} 08:53:17?}
        \item The Hound of the Baskervilles (1901--1902), {\color{red} 06:10:32?}
        }
    \end{enumerate}
    \item STAGE 1: TOTAL approx 36 hours if 16 hours LibriSpeech listen + 20 hours Sherlock books 1--3 (\textbf{NB: could bump to 40 hours as proposed to MRC if include all dev-clean...})
    \item STAGE 2: TOTAL approx 50 hours if 16 hours LibriSpeech listen + 34 hours Sherlock books 1--5
    \item STAGE 3: \textbf{TOTAL approx 60 hours if 36 hours LibriSpeech listen + 34 hours Sherlock books 1--5 (about equal amounts from each)} NB not counting additional 36 hours LibriSpeech think for PNPL Gold...
    
    {\color{purple}
    \item For v2?
    \begin{itemize}
        \item 64 hrs listen (60 hrs train) from 64 subjects? (120 hrs total -- for TRAIN, with additional TEST)
        \item (not counting 64 additional hours think (60 hrs train) from the same 64 subjects?)
        \item dev/val data all from same set?
        \item half test set from 64 subjects same, half sampled from full test set? or all test sampled?
    \end{itemize}
    }
%%%
    \item {\color{green} OLD OLD OLD OLD OLD}
    \item Start with sherlock3, to sanity check against Armeni
    \item All sherlock books that were in the public domain at the time; all 4 novels (Study, Sign, Hound, Valley) and 4/5 collections of short stories (Adventures, Memoirs, Return, Last Bow; only excluding The Case-Book of Sherlock Holmes, 1927, which was the last to be released to the public domain, in XXX in the UK (XXX in the US) and did not have a LibriVox recording by the same narrator at the time of the experiment). %use different narrator?
    \item All Sherlock Holmes read by David Clarke and distributed through the LibriVox public library (\url{https://librivox.org}). 
    \item Text retrieved from \url{XXX} and manually corrected to match the audio (when divergences) and text normalised (e.g.~numbers converted to text)%give example from TextGrid
    \item {\color{red} NB times below from LibriVox website (total = 60 hours 13 minutes 10 seconds) -> TODO: check actual play time of all files....}
    \begin{enumerate}
        \item A Study in Scarlet (1887), {\color{red} 04:37:34?}
        \item The Sign of the Four (1890), {\color{red} 4:27:31?}
        \item The Hound of the Baskervilles (1901--1902), {\color{red} 06:10:32?}
        \item The Valley of Fear (1914--1915), {\color{red} 06:06:17?}
        \item The Adventures of Sherlock Holmes (1892), {\color{blue} 12 stories}, {\color{red} 10:56:13?}
        \item The Memoirs of Sherlock Holmes (1893--1894), {\color{blue} 12 stories}, {\color{red} 08:53:17?}
        \item The Return of Sherlock Holmes (1905), {\color{blue} 13 stories}, {\color{red} 11:51:17?}
        \item His Last Bow (1917), {\color{blue} 7 stories}, {\color{red} 07:10:29?}
        \item $\text{\sout{The Case-Book of Sherlock Holmes (1927),  {\color{blue} 12 stories}}}$
    \end{enumerate}
    \item Comprehension questions (multiple choice) after each chapter (different than in covert reading version) %3 questions per chapter? Birtan
    \item Selection of audio (different speakers) from LibriSpeech {\color{red} 40 hours worth? for a total of 100 hrs within subject data}? / use in PNPL-Gold?
    \begin{itemize}
        \item 
    \end{itemize}
\end{itemize}
